InferFix: End-to-End Program Repair with LLMs

Software development life cycle is profoundly influenced by bugs: their introduction, identification, and eventual resolution account for a significant portion of software cost. This has motivated software engineering researchers and practitioners to propose different approaches for automating the identification and repair of software defects. Large language models have been adapted to the program repair task through few-shot demonstration learning and instruction prompting, treating this as an infilling task. However, these models have only focused on learning general bug-fixing patterns for uncategorized bugs mined from public repositories. In this paper, we propose InferFix: a transformer-based program repair framework paired with a state-of-the-art static analyzer to fix critical security and performance bugs. InferFix combines a Retriever -- transformer encoder model pretrained via contrastive learning objective, which aims at searching for semantically equivalent bugs and corresponding fixes; and a Generator -- a large language model (Codex Cushman) finetuned on supervised bug-fix data with prompts augmented via bug type annotations and semantically similar fixes retrieved from an external non-parametric memory. To train and evaluate our approach, we curated InferredBugs, a novel, metadata-rich dataset of bugs extracted by executing the Infer static analyzer on the change histories of thousands of Java and C# repositories. Our evaluation demonstrates that InferFix outperforms strong LLM baselines, with a top-1 accuracy of 65.6% for generating fixes in C# and 76.8% in Java. We discuss the deployment of InferFix alongside Infer at Microsoft which offers an end-to-end solution for detection, classification, and localization of bugs, as well as fixing and validation of candidate patches, integrated in the continuous integration pipeline to automate the software development workflow.

==> dataset.tex <==
\subsection{Null Dereference Examples}

%\inputminted{java}{code_examples/null1_before.java}
%\inputminted{java}{code_examples/null1_after.java}

In this example from the java-bigtable-hbase repository, commit 708b8e8a9eeecfab17ad05a036880c467c42674c resolves the below issue in which status.getDescription() can be null.

\begin{minted}[breaklines,breakanywhere]{java}
@Override
public void onClose(Status status, Metadata trailers) {
if (status.getCode() == Status.Code.CANCELLED
    && status.getDescription().contains(TIMEOUT_CANCEL_MSG)) {
  // If this was canceled because of handleTimeout(). The cancel is immediately retried or
  // completed in another fashion.
  return;
}
super.onClose(status, trailers);
}
\end{minted}

\begin{minted}[highlightlines={4},breaklines,breakanywhere]{java}
@Override
public void onClose(Status status, Metadata trailers) {
if (status.getCode() == Status.Code.CANCELLED
    && status.getDescription() != null
    && status.getDescription().contains(TIMEOUT_CANCEL_MSG)) {
  // If this was canceled because of handleTimeout(). The cancel is immediately retried or
  // completed in another fashion.
  return;
}
super.onClose(status, trailers);
}
\end{minted}

In this example from jackson-databind repository, commit 0ee6a6d2a1739e48870d6f26a5a217382c807798 removes a dereference which was causing a null pointer description. 

\begin{minted}[breaklines,breakanywhere]{java}
@Override
public PropertyMetadata getMetadata() {
  final Boolean b = _findRequired();
  final String desc = _findDescription();
  final Integer idx = _findIndex();
  final String def = _findDefaultValue();
  if (b == null && idx == null && def == null) {
    return (desc == null) ? PropertyMetadata.STD_REQUIRED_OR_OPTIONAL
      : PropertyMetadata.STD_REQUIRED_OR_OPTIONAL.withDescription(desc);
  }
  return PropertyMetadata.construct(b.booleanValue(), desc, idx, def);
}
\end{minted}

\begin{minted}[highlightlines={11},breaklines,breakanywhere]{java}
@Override
public PropertyMetadata getMetadata() {
  final Boolean b = _findRequired();
  final String desc = _findDescription();
  final Integer idx = _findIndex();
  final String def = _findDefaultValue();
  if (b == null && idx == null && def == null) {
    return (desc == null) ? PropertyMetadata.STD_REQUIRED_OR_OPTIONAL
      : PropertyMetadata.STD_REQUIRED_OR_OPTIONAL.withDescription(desc);
  }
  return PropertyMetadata.construct(b, desc, idx, def);
}
\end{minted}

\subsection{Resource Leak Examples}

In this example from OSM2World, commit 8d7a479714cb2dda
448a2520aeab6252b1ab96f2 closes Bufferedreader reader, which hadn't been closed:

\begin{minted}[breaklines,breakanywhere]{java}
public static final boolean isJOSMGenerated(File file) {
	
  try {
		
    BufferedReader reader = new BufferedReader(new FileReader(file));
		
    for (int i=0; i<100; i++) {
      String line = reader.readLine();
      if (line != null) {
        if (line.contains("generator='JOSM'")) {
          return true;
        }
      }
    }
		
    reader.close();
		
  } catch (IOException e) { }
	
  return false;
	
}
\end{minted}

\begin{minted}[highlightlines={11},breaklines,breakanywhere]{java}
public static final boolean isJOSMGenerated(File file) {
	
  try {
		
    BufferedReader reader = new BufferedReader(new FileReader(file));
		
    for (int i=0; i<100; i++) {
      String line = reader.readLine();
      if (line != null) {
        if (line.contains("generator='JOSM'")) {
          reader.close();
          return true;
        }
      }
    }
		
    reader.close();
		
  } catch (IOException e) { }
	
  return false;
	
}
\end{minted}

\noindent In this example from urlbuilder, commit 7ef505684e2a7b1c860
df7a78c8d91217147f464 removes reader's final keyword and closes it:

\begin{minted}[breaklines,breakanywhere]{java}
private static String readResource(final String name) {
    final StringBuilder ret = new StringBuilder();
    InputStream is = null;
    try {
        is = UrlRegularExpressions.class.getClassLoader().getResourceAsStream(name);
        final InputStreamReader reader = new InputStreamReader(is, ASCII);
        int read = 0;
        final char[] buf = new char[1024];
        do {
            read = reader.read(buf, 0, buf.length);
            if (read > 0) {
                ret.append(buf, 0, read);
            }
        } while (read >= 0);
    } catch (final IOException ex) {
        throw new RuntimeException(ex);
    } finally {
        closeQuietly(is);
    }
    return ret.toString();
}
\end{minted}

\begin{minted}[highlightlines={4,7,20},breaklines,breakanywhere]{java}
private static String readResource(final String name) {
    final StringBuilder ret = new StringBuilder();
    InputStream is = null;
    InputStreamReader reader = null;
    try {
        is = UrlRegularExpressions.class.getClassLoader().getResourceAsStream(name);
        reader = new InputStreamReader(is, ASCII);
        int read = 0;
        final char[] buf = new char[1024];
        do {
            read = reader.read(buf, 0, buf.length);
            if (read > 0) {
                ret.append(buf, 0, read);
            }
        } while (read >= 0);
    } catch (final IOException ex) {
        throw new RuntimeException(ex);
    } finally {
        closeQuietly(is);
        closeQuietly(reader);
    }
    return ret.toString();
}
\end{minted}
